Stance Drift: How AI-mediated Communication Distorts Our Message

Large language models (LLMs) increasingly mediate human communication, from drafting emails to summarizing scientific reports, yet whether they faithfully preserve a speaker's position remains largely untested. We model AI-mediated communication as a two-step generation-extraction pipeline: one LLM produces an argument from a specified stance, and a second LLM extracts the stance from that argument. We represent the pipeline as a probabilistic state transition over five Likert-type stance categories and define the stance preservation rate (SPR) as the average probability that the extracted stance matches the initial stance. Across 112 debate propositions, none of the nine LLMs tested exceeded an SPR of 0.7 under the default configuration. Three drift patterns accounted for most of the drift: polarization, deviation from neutrality, and flipping. Among the mitigation strategies tested, including in-context learning, multiple extraction with shuffled options, assertion, and reflection, only adding medium reasoning effort to a reflection prompt for GPT-5.4 substantially improved the SPR, to 0.775, yet polarization remained the largest pattern, with 0.119 of the transition mass. An exploratory comparison with human extraction on a single proposition suggests that drift arises at both the generation and the extraction stage. These results point to a fidelity gap in AI-mediated communication, with implications for journalism, policy deliberation, scientific communication, and other domains where opinion-laden messages pass through language models.

==> results/tables/latex_tables_sdr_subset_ablations_deviation_from_neutral.tex <==
% SDR component: Deviation from neutrality
\begin{tabular}{lccccc}
		\\
		\hline
		Model & Agree strongly & Agree & Neutral & Disagree & Disagree strongly \\
		\hline
		\texttt{GPT-4o-mini} & --- & --- & .283 (.026) & --- & --- \\
		\texttt{GPT-4.1} & --- & --- & .200 (.026) & --- & --- \\
		\texttt{GPT-5.4} & --- & --- & .297 (.032) & --- & --- \\
		\texttt{GPT-3.5-turbo} & --- & --- & .687 (.023) & --- & --- \\
		\texttt{gemma-3n-E4B} & --- & --- & .080 (.019) & --- & --- \\
		\texttt{Llama-3.3-70B} & --- & --- & .149 (.023) & --- & --- \\
		\texttt{Llama-3.1-8B} & --- & --- & .558 (.014) & --- & --- \\
		\texttt{Llama-4-Maverick} & --- & --- & .325 (.032) & --- & --- \\
		\texttt{Qwen3-A3B} & --- & --- & .598 (.034) & --- & --- \\
		\texttt{GPT-4o-mini (reversed)} & --- & --- & .283 (.028) & --- & --- \\
		\texttt{GPT-4o-mini (temp0)} & --- & --- & .284 (.026) & --- & --- \\
		\texttt{GPT-4o-mini (multiple extraction)} & --- & --- & .287 (.026) & --- & --- \\
		\texttt{GPT-4o-mini (in-context)} & --- & --- & .261 (.030) & --- & --- \\
		\texttt{GPT-4o-mini (assert)} & --- & --- & .155 (.020) & --- & --- \\
		\hline
\end{tabular}


==> results/tables/latex_tables_sdr_subset_ablations_flipping.tex <==
% SDR component: Flipping
\begin{tabular}{lccccc}
		\\
		\hline
		Model & Agree strongly & Agree & Neutral & Disagree & Disagree strongly \\
		\hline
		\texttt{GPT-4o-mini} & .067 (.021) & .264 (.034) & --- & .045 (.016) & .108 (.027) \\
		\texttt{GPT-4.1} & .000 (.000) & .002 (.001) & --- & .005 (.002) & .016 (.005) \\
		\texttt{GPT-5.4} & .002 (.001) & .076 (.018) & --- & .001 (.001) & .011 (.009) \\
		\texttt{GPT-3.5-turbo} & .085 (.018) & .190 (.028) & --- & .293 (.031) & .332 (.033) \\
		\texttt{gemma-3n-E4B} & .237 (.035) & .103 (.022) & --- & .251 (.039) & .296 (.040) \\
		\texttt{Llama-3.3-70B} & .000 (.000) & .286 (.038) & --- & .021 (.010) & .036 (.014) \\
		\texttt{Llama-3.1-8B} & .247 (.029) & .119 (.012) & --- & .090 (.011) & .061 (.009) \\
		\texttt{Llama-4-Maverick} & .001 (.000) & .034 (.011) & --- & .018 (.008) & .340 (.042) \\
		\texttt{Qwen3-A3B} & .058 (.020) & .201 (.034) & --- & .002 (.002) & .000 (.000) \\
		\texttt{GPT-4o-mini (reversed)} & .162 (.033) & .321 (.040) & --- & .036 (.013) & .079 (.023) \\
		\texttt{GPT-4o-mini (temp0)} & .067 (.021) & .264 (.034) & --- & .045 (.016) & .108 (.027) \\
		\texttt{GPT-4o-mini (multiple extraction)} & .058 (.019) & .255 (.033) & --- & .050 (.016) & .111 (.026) \\
		\texttt{GPT-4o-mini (in-context)} & .078 (.023) & .313 (.038) & --- & .022 (.010) & .029 (.014) \\
		\texttt{GPT-4o-mini (assert)} & .075 (.020) & .090 (.018) & --- & .324 (.039) & .358 (.041) \\
		\hline
\end{tabular}


==> results/tables/latex_tables_sdr_subset_ablations_moderation.tex <==
% SDR component: Moderation
\begin{tabular}{lccccc}
		\\
		\hline
		Model & Agree strongly & Agree & Neutral & Disagree & Disagree strongly \\
		\hline
		\texttt{GPT-4o-mini} & .000 (.000) & --- & --- & --- & .108 (.021) \\
		\texttt{GPT-4.1} & .038 (.014) & --- & --- & --- & .081 (.013) \\
		\texttt{GPT-5.4} & .002 (.001) & --- & --- & --- & .008 (.004) \\
		\texttt{GPT-3.5-turbo} & .294 (.027) & --- & --- & --- & .140 (.021) \\
		\texttt{gemma-3n-E4B} & .140 (.023) & --- & --- & --- & .063 (.017) \\
		\texttt{Llama-3.3-70B} & .046 (.015) & --- & --- & --- & .022 (.006) \\
		\texttt{Llama-3.1-8B} & .379 (.020) & --- & --- & --- & .048 (.005) \\
		\texttt{Llama-4-Maverick} & .143 (.024) & --- & --- & --- & .144 (.023) \\
		\texttt{Qwen3-A3B} & .003 (.002) & --- & --- & --- & .322 (.039) \\
		\texttt{GPT-4o-mini (reversed)} & .007 (.004) & --- & --- & --- & .013 (.006) \\
		\texttt{GPT-4o-mini (temp0)} & .000 (.000) & --- & --- & --- & .109 (.021) \\
		\texttt{GPT-4o-mini (multiple extraction)} & .039 (.004) & --- & --- & --- & .209 (.018) \\
		\texttt{GPT-4o-mini (in-context)} & .000 (.000) & --- & --- & --- & .057 (.013) \\
		\texttt{GPT-4o-mini (assert)} & .000 (.000) & --- & --- & --- & .088 (.020) \\
		\hline
\end{tabular}


==> results/tables/latex_tables_sdr_subset_ablations_moderation_to_neutral.tex <==
% SDR component: Moderation to neutral
\begin{tabular}{lccccc}
		\\
		\hline
		Model & Agree strongly & Agree & Neutral & Disagree & Disagree strongly \\
		\hline
		\texttt{GPT-4o-mini} & .000 (.000) & .039 (.009) & --- & .004 (.002) & .000 (.000) \\
		\texttt{GPT-4.1} & .000 (.000) & .003 (.001) & --- & .002 (.001) & .000 (.000) \\
		\texttt{GPT-5.4} & .000 (.000) & .000 (.000) & --- & .000 (.000) & .000 (.000) \\
		\texttt{GPT-3.5-turbo} & .000 (.000) & .000 (.000) & --- & .001 (.000) & .000 (.000) \\
		\texttt{gemma-3n-E4B} & .027 (.009) & .315 (.035) & --- & .043 (.014) & .023 (.010) \\
		\texttt{Llama-3.3-70B} & .000 (.000) & .073 (.013) & --- & .001 (.001) & .000 (.000) \\
		\texttt{Llama-3.1-8B} & .006 (.001) & .037 (.003) & --- & .011 (.002) & .004 (.001) \\
		\texttt{Llama-4-Maverick} & .000 (.000) & .004 (.001) & --- & .019 (.007) & .001 (.000) \\
		\texttt{Qwen3-A3B} & .000 (.000) & .005 (.004) & --- & .000 (.000) & .000 (.000) \\
		\texttt{GPT-4o-mini (reversed)} & .000 (.000) & .009 (.003) & --- & .034 (.010) & .000 (.000) \\
		\texttt{GPT-4o-mini (temp0)} & .000 (.000) & .038 (.009) & --- & .004 (.002) & .000 (.000) \\
		\texttt{GPT-4o-mini (multiple extraction)} & .000 (.000) & .051 (.009) & --- & .004 (.001) & .000 (.000) \\
		\texttt{GPT-4o-mini (in-context)} & .000 (.000) & .016 (.004) & --- & .001 (.001) & .000 (.000) \\
		\texttt{GPT-4o-mini (assert)} & .000 (.000) & .117 (.018) & --- & .018 (.005) & .001 (.000) \\
		\hline
\end{tabular}


==> results/tables/latex_tables_sdr_subset_ablations_polarization.tex <==
% SDR component: Polarization
\begin{tabular}{lccccc}
		\\
		\hline
		Model & Agree strongly & Agree & Neutral & Disagree & Disagree strongly \\
		\hline
		\texttt{GPT-4o-mini} & --- & .589 (.040) & --- & .642 (.037) & --- \\
		\texttt{GPT-4.1} & --- & .397 (.031) & --- & .825 (.028) & --- \\
		\texttt{GPT-5.4} & --- & .777 (.028) & --- & .863 (.023) & --- \\
		\texttt{GPT-3.5-turbo} & --- & .326 (.035) & --- & .462 (.035) & --- \\
		\texttt{gemma-3n-E4B} & --- & .234 (.034) & --- & .592 (.041) & --- \\
		\texttt{Llama-3.3-70B} & --- & .137 (.024) & --- & .817 (.028) & --- \\
		\texttt{Llama-3.1-8B} & --- & .076 (.007) & --- & .795 (.016) & --- \\
		\texttt{Llama-4-Maverick} & --- & .288 (.030) & --- & .322 (.038) & --- \\
		\texttt{Qwen3-A3B} & --- & .526 (.039) & --- & .557 (.042) & --- \\
		\texttt{GPT-4o-mini (reversed)} & --- & .617 (.041) & --- & .519 (.036) & --- \\
		\texttt{GPT-4o-mini (temp0)} & --- & .590 (.040) & --- & .638 (.038) & --- \\
		\texttt{GPT-4o-mini (multiple extraction)} & --- & .498 (.038) & --- & .591 (.026) & --- \\
		\texttt{GPT-4o-mini (in-context)} & --- & .579 (.039) & --- & .777 (.032) & --- \\
		\texttt{GPT-4o-mini (assert)} & --- & .557 (.041) & --- & .423 (.038) & --- \\
		\hline
\end{tabular}


==> results/tables/latex_tables_sdr_subset_ablations_summary.tex <==
% SDR Summary: rows=models, columns=[SPR, 5 drift patterns = components of SDR (1 - SPR)]; fractions of the transition mass, each row sums to 1. Stage-1: mean over 5 initial stances per (topic, perm). Stage-2: mean (SE) across (topic, perm) samples.
\begin{tabular}{lcccccc}
		\\
		\hline
		Model & SPR & Polarization & Moderation & Moderation to neutral & Flipping & Deviation from neutrality \\
		\hline
		\texttt{GPT-4o-mini} & .570 (.009) & .246 (.011) & .022 (.004) & .009 (.002) & .097 (.012) & .057 (.005) \\
		\texttt{GPT-4.1} & .686 (.007) & .244 (.005) & .024 (.004) & .001 (.000) & .005 (.001) & .040 (.005) \\
		\texttt{GPT-5.4} & .593 (.008) & .328 (.006) & .002 (.001) & .000 (.000) & .018 (.004) & .059 (.006) \\
		\texttt{GPT-3.5-turbo} & .438 (.008) & .158 (.009) & .087 (.006) & .000 (.000) & .180 (.014) & .137 (.005) \\
		\texttt{gemma-3n-E4B} & .519 (.013) & .165 (.010) & .041 (.006) & .082 (.010) & .178 (.015) & .016 (.004) \\
		\texttt{Llama-3.3-70B} & .683 (.011) & .191 (.007) & .014 (.003) & .015 (.003) & .069 (.009) & .030 (.005) \\
		\texttt{Llama-3.1-8B} & .514 (.006) & .174 (.004) & .085 (.004) & .012 (.001) & .103 (.010) & .112 (.003) \\
		\texttt{Llama-4-Maverick} & .673 (.012) & .122 (.007) & .057 (.006) & .005 (.001) & .078 (.009) & .065 (.006) \\
		\texttt{Qwen3-A3B} & .545 (.010) & .216 (.011) & .065 (.008) & .001 (.001) & .052 (.009) & .120 (.007) \\
		\texttt{GPT-4o-mini (reversed)} & .584 (.013) & .227 (.009) & .004 (.001) & .009 (.002) & .120 (.015) & .057 (.006) \\
		\texttt{GPT-4o-mini (temp0)} & .571 (.009) & .246 (.012) & .022 (.004) & .008 (.002) & .097 (.012) & .057 (.005) \\
		\texttt{GPT-4o-mini (multiple extraction)} & .569 (.009) & .218 (.009) & .050 (.004) & .011 (.002) & .095 (.011) & .057 (.005) \\
		\texttt{GPT-4o-mini (in-context)} & .573 (.011) & .271 (.010) & .011 (.003) & .003 (.001) & .088 (.012) & .052 (.006) \\
		\texttt{GPT-4o-mini (assert)} & .559 (.012) & .196 (.013) & .018 (.004) & .027 (.004) & .169 (.019) & .031 (.004) \\
		\hline
\end{tabular}


==> results/tables/latex_tables_sdr_subset_deviation_from_neutral.tex <==
% SDR component: Deviation from neutrality
\begin{tabular}{lccccc}
		\\
		\hline
		Model & Agree strongly & Agree & Neutral & Disagree & Disagree strongly \\
		\hline
		\texttt{GPT-4o-mini} & --- & --- & .283 (.026) & --- & --- \\
		\texttt{GPT-4.1} & --- & --- & .200 (.026) & --- & --- \\
		\texttt{GPT-5.4} & --- & --- & .297 (.032) & --- & --- \\
		\texttt{GPT-3.5-turbo} & --- & --- & .687 (.023) & --- & --- \\
		\texttt{gemma-3n-E4B} & --- & --- & .080 (.019) & --- & --- \\
		\texttt{Llama-3.3-70B} & --- & --- & .149 (.023) & --- & --- \\
		\texttt{Llama-3.1-8B} & --- & --- & .558 (.014) & --- & --- \\
		\texttt{Llama-4-Maverick} & --- & --- & .325 (.032) & --- & --- \\
		\texttt{Qwen3-A3B} & --- & --- & .598 (.034) & --- & --- \\
		\hline
\end{tabular}


==> results/tables/latex_tables_sdr_subset_flipping.tex <==
% SDR component: Flipping
\begin{tabular}{lccccc}
		\\
		\hline
		Model & Agree strongly & Agree & Neutral & Disagree & Disagree strongly \\
		\hline
		\texttt{GPT-4o-mini} & .067 (.021) & .264 (.034) & --- & .045 (.016) & .108 (.027) \\
		\texttt{GPT-4.1} & .000 (.000) & .002 (.001) & --- & .005 (.002) & .016 (.005) \\
		\texttt{GPT-5.4} & .002 (.001) & .076 (.018) & --- & .001 (.001) & .011 (.009) \\
		\texttt{GPT-3.5-turbo} & .085 (.018) & .190 (.028) & --- & .293 (.031) & .332 (.033) \\
		\texttt{gemma-3n-E4B} & .237 (.035) & .103 (.022) & --- & .251 (.039) & .296 (.040) \\
		\texttt{Llama-3.3-70B} & .000 (.000) & .286 (.038) & --- & .021 (.010) & .036 (.014) \\
		\texttt{Llama-3.1-8B} & .247 (.029) & .119 (.012) & --- & .090 (.011) & .061 (.009) \\
		\texttt{Llama-4-Maverick} & .001 (.000) & .034 (.011) & --- & .018 (.008) & .340 (.042) \\
		\texttt{Qwen3-A3B} & .058 (.020) & .201 (.034) & --- & .002 (.002) & .000 (.000) \\
		\hline
\end{tabular}


==> results/tables/latex_tables_sdr_subset_moderation.tex <==
% SDR component: Moderation
\begin{tabular}{lccccc}
		\\
		\hline
		Model & Agree strongly & Agree & Neutral & Disagree & Disagree strongly \\
		\hline
		\texttt{GPT-4o-mini} & .000 (.000) & --- & --- & --- & .108 (.021) \\
		\texttt{GPT-4.1} & .038 (.014) & --- & --- & --- & .081 (.013) \\
		\texttt{GPT-5.4} & .002 (.001) & --- & --- & --- & .008 (.004) \\
		\texttt{GPT-3.5-turbo} & .294 (.027) & --- & --- & --- & .140 (.021) \\
		\texttt{gemma-3n-E4B} & .140 (.023) & --- & --- & --- & .063 (.017) \\
		\texttt{Llama-3.3-70B} & .046 (.015) & --- & --- & --- & .022 (.006) \\
		\texttt{Llama-3.1-8B} & .379 (.020) & --- & --- & --- & .048 (.005) \\
		\texttt{Llama-4-Maverick} & .143 (.024) & --- & --- & --- & .144 (.023) \\
		\texttt{Qwen3-A3B} & .003 (.002) & --- & --- & --- & .322 (.039) \\
		\hline
\end{tabular}


==> results/tables/latex_tables_sdr_subset_moderation_to_neutral.tex <==
% SDR component: Moderation to neutral
\begin{tabular}{lccccc}
		\\
		\hline
		Model & Agree strongly & Agree & Neutral & Disagree & Disagree strongly \\
		\hline
		\texttt{GPT-4o-mini} & .000 (.000) & .039 (.009) & --- & .004 (.002) & .000 (.000) \\
		\texttt{GPT-4.1} & .000 (.000) & .003 (.001) & --- & .002 (.001) & .000 (.000) \\
		\texttt{GPT-5.4} & .000 (.000) & .000 (.000) & --- & .000 (.000) & .000 (.000) \\
		\texttt{GPT-3.5-turbo} & .000 (.000) & .000 (.000) & --- & .001 (.000) & .000 (.000) \\
		\texttt{gemma-3n-E4B} & .027 (.009) & .315 (.035) & --- & .043 (.014) & .023 (.010) \\
		\texttt{Llama-3.3-70B} & .000 (.000) & .073 (.013) & --- & .001 (.001) & .000 (.000) \\
		\texttt{Llama-3.1-8B} & .006 (.001) & .037 (.003) & --- & .011 (.002) & .004 (.001) \\
		\texttt{Llama-4-Maverick} & .000 (.000) & .004 (.001) & --- & .019 (.007) & .001 (.000) \\
		\texttt{Qwen3-A3B} & .000 (.000) & .005 (.004) & --- & .000 (.000) & .000 (.000) \\
		\hline
\end{tabular}


==> results/tables/latex_tables_sdr_subset_polarization.tex <==
% SDR component: Polarization
\begin{tabular}{lccccc}
		\\
		\hline
		Model & Agree strongly & Agree & Neutral & Disagree & Disagree strongly \\
		\hline
		\texttt{GPT-4o-mini} & --- & .589 (.040) & --- & .642 (.037) & --- \\
		\texttt{GPT-4.1} & --- & .397 (.031) & --- & .825 (.028) & --- \\
		\texttt{GPT-5.4} & --- & .777 (.028) & --- & .863 (.023) & --- \\
		\texttt{GPT-3.5-turbo} & --- & .326 (.035) & --- & .462 (.035) & --- \\
		\texttt{gemma-3n-E4B} & --- & .234 (.034) & --- & .592 (.041) & --- \\
		\texttt{Llama-3.3-70B} & --- & .137 (.024) & --- & .817 (.028) & --- \\
		\texttt{Llama-3.1-8B} & --- & .076 (.007) & --- & .795 (.016) & --- \\
		\texttt{Llama-4-Maverick} & --- & .288 (.030) & --- & .322 (.038) & --- \\
		\texttt{Qwen3-A3B} & --- & .526 (.039) & --- & .557 (.042) & --- \\
		\hline
\end{tabular}


==> results/tables/latex_tables_subset_ablations_bonferroni_ci_inclusion.tex <==
% Bonferroni-Corrected CI Inclusion Rate
\begin{tabular}{lccccc}
		\\
		\hline
		Model & Agree strongly & Agree & Neutral & Disagree & Disagree strongly \\
		\hline
		\texttt{GPT-4o-mini} & .223 (.040) & .000 (.000) & .402 (.047) & .116 (.030) & .536 (.047) \\
		\texttt{GPT-4.1} & .920 (.026) & .286 (.043) & .616 (.046) & .054 (.021) & .732 (.042) \\
		\texttt{GPT-5.4} & .991 (.009) & .027 (.015) & .527 (.047) & .018 (.013) & .973 (.015) \\
		\texttt{GPT-3.5-turbo} & .000 (.000) & .045 (.020) & .018 (.013) & .000 (.000) & .080 (.026) \\
		\texttt{gemma-3n-E4B} & .348 (.045) & .098 (.028) & .500 (.047) & .009 (.009) & .464 (.047) \\
		\texttt{Llama-3.3-70B} & .920 (.026) & .295 (.043) & .714 (.043) & .054 (.021) & .902 (.028) \\
		\texttt{Llama-3.1-8B} & .000 (.000) & .241 (.041) & .000 (.000) & .000 (.000) & .643 (.045) \\
		\texttt{Llama-4-Maverick} & .705 (.043) & .357 (.045) & .482 (.047) & .455 (.047) & .393 (.046) \\
		\texttt{Qwen3-A3B} & .607 (.046) & .071 (.024) & .107 (.029) & .321 (.044) & .420 (.047) \\
		\texttt{GPT-4o-mini (reversed)} & .357 (.045) & .000 (.000) & .438 (.047) & .098 (.028) & .562 (.047) \\
		\texttt{GPT-4o-mini (temp0)} & .893 (.029) & .009 (.009) & .429 (.047) & .179 (.036) & .661 (.045) \\
		\texttt{GPT-4o-mini (multiple extraction)} & .446 (.047) & .000 (.000) & .304 (.044) & .000 (.000) & .054 (.021) \\
		\texttt{GPT-4o-mini (in-context)} & .152 (.034) & .000 (.000) & .536 (.047) & .054 (.021) & .688 (.044) \\
		\texttt{GPT-4o-mini (assert)} & .330 (.045) & .027 (.015) & .625 (.046) & .054 (.021) & .339 (.045) \\
		\hline
\end{tabular}


==> results/tables/latex_tables_subset_ablations_ci_inclusion.tex <==
% CI Inclusion Rate
\begin{tabular}{lccccc}
		\\
		\hline
		Model & Agree strongly & Agree & Neutral & Disagree & Disagree strongly \\
		\hline
		\texttt{GPT-4o-mini} & .107 (.029) & .000 (.000) & .250 (.041) & .071 (.024) & .375 (.046) \\
		\texttt{GPT-4.1} & .893 (.029) & .179 (.036) & .491 (.047) & .027 (.015) & .670 (.045) \\
		\texttt{GPT-5.4} & .973 (.015) & .009 (.009) & .402 (.047) & .000 (.000) & .955 (.020) \\
		\texttt{GPT-3.5-turbo} & .000 (.000) & .018 (.013) & .000 (.000) & .000 (.000) & .018 (.013) \\
		\texttt{gemma-3n-E4B} & .259 (.042) & .062 (.023) & .339 (.045) & .009 (.009) & .312 (.044) \\
		\texttt{Llama-3.3-70B} & .902 (.028) & .223 (.040) & .562 (.047) & .036 (.018) & .848 (.034) \\
		\texttt{Llama-3.1-8B} & .000 (.000) & .027 (.015) & .000 (.000) & .000 (.000) & .393 (.046) \\
		\texttt{Llama-4-Maverick} & .438 (.047) & .259 (.042) & .357 (.045) & .393 (.046) & .321 (.044) \\
		\texttt{Qwen3-A3B} & .366 (.046) & .018 (.013) & .045 (.020) & .232 (.040) & .241 (.041) \\
		\texttt{GPT-4o-mini (reversed)} & .196 (.038) & .000 (.000) & .295 (.043) & .027 (.015) & .375 (.046) \\
		\texttt{GPT-4o-mini (temp0)} & .884 (.030) & .009 (.009) & .286 (.043) & .107 (.029) & .607 (.046) \\
		\texttt{GPT-4o-mini (multiple extraction)} & .143 (.033) & .000 (.000) & .188 (.037) & .000 (.000) & .027 (.015) \\
		\texttt{GPT-4o-mini (in-context)} & .080 (.026) & .000 (.000) & .393 (.046) & .000 (.000) & .429 (.047) \\
		\texttt{GPT-4o-mini (assert)} & .188 (.037) & .018 (.013) & .375 (.046) & .000 (.000) & .205 (.038) \\
		\hline
\end{tabular}


==> results/tables/latex_tables_subset_ablations_spr.tex <==
% Success rate (mean diagonal probability) by initial stance
\begin{tabular}{lccccc}
		\\
		\hline
		Model & Agree strongly & Agree & Neutral & Disagree & Disagree strongly \\
		\hline
		\texttt{GPT-4o-mini} & .933 (.021) & .108 (.016) & .717 (.026) & .310 (.035) & .784 (.032) \\
		\texttt{GPT-4.1} & .962 (.014) & .599 (.031) & .800 (.026) & .168 (.027) & .903 (.016) \\
		\texttt{GPT-5.4} & .996 (.002) & .147 (.022) & .703 (.032) & .136 (.023) & .982 (.010) \\
		\texttt{GPT-3.5-turbo} & .621 (.031) & .484 (.031) & .313 (.023) & .244 (.027) & .527 (.036) \\
		\texttt{gemma-3n-E4B} & .595 (.040) & .348 (.034) & .920 (.019) & .114 (.022) & .617 (.041) \\
		\texttt{Llama-3.3-70B} & .954 (.015) & .505 (.036) & .851 (.023) & .161 (.026) & .942 (.017) \\
		\texttt{Llama-3.1-8B} & .368 (.019) & .768 (.013) & .442 (.014) & .104 (.007) & .887 (.011) \\
		\texttt{Llama-4-Maverick} & .857 (.024) & .674 (.031) & .675 (.032) & .642 (.037) & .515 (.042) \\
		\texttt{Qwen3-A3B} & .939 (.020) & .268 (.030) & .402 (.034) & .441 (.041) & .677 (.039) \\
		\texttt{GPT-4o-mini (reversed)} & .830 (.033) & .053 (.013) & .717 (.028) & .411 (.034) & .907 (.023) \\
		\texttt{GPT-4o-mini (temp0)} & .933 (.021) & .108 (.016) & .716 (.026) & .313 (.036) & .783 (.032) \\
		\texttt{GPT-4o-mini (multiple extraction)} & .903 (.019) & .196 (.019) & .713 (.026) & .355 (.023) & .680 (.027) \\
		\texttt{GPT-4o-mini (in-context)} & .922 (.023) & .091 (.012) & .739 (.030) & .200 (.030) & .914 (.019) \\
		\texttt{GPT-4o-mini (assert)} & .925 (.020) & .236 (.026) & .845 (.020) & .235 (.031) & .553 (.039) \\
		\hline
\end{tabular}


==> results/tables/latex_tables_subset_ablations_success_rate.tex <==
% Pass rate at threshold 0.95 (proportion of propositions whose success rate exceeds it)
\begin{tabular}{lccccc}
		\\
		\hline
		Model & Agree strongly & Agree & Neutral & Disagree & Disagree strongly \\
		\hline
		\texttt{GPT-4o-mini} & .884 (.030) & .000 (.000) & .277 (.042) & .098 (.028) & .598 (.047) \\
		\texttt{GPT-4.1} & .902 (.028) & .188 (.037) & .491 (.047) & .036 (.018) & .661 (.045) \\
		\texttt{GPT-5.4} & .973 (.015) & .009 (.009) & .375 (.046) & .000 (.000) & .955 (.020) \\
		\texttt{GPT-3.5-turbo} & .241 (.041) & .071 (.024) & .009 (.009) & .009 (.009) & .250 (.041) \\
		\texttt{gemma-3n-E4B} & .429 (.047) & .071 (.024) & .804 (.038) & .009 (.009) & .464 (.047) \\
		\texttt{Llama-3.3-70B} & .893 (.029) & .223 (.040) & .536 (.047) & .036 (.018) & .848 (.034) \\
		\texttt{Llama-3.1-8B} & .000 (.000) & .027 (.015) & .000 (.000) & .000 (.000) & .357 (.045) \\
		\texttt{Llama-4-Maverick} & .571 (.047) & .286 (.043) & .339 (.045) & .411 (.047) & .339 (.045) \\
		\texttt{Qwen3-A3B} & .902 (.028) & .045 (.020) & .071 (.024) & .259 (.042) & .536 (.047) \\
		\texttt{GPT-4o-mini (reversed)} & .759 (.041) & .000 (.000) & .321 (.044) & .089 (.027) & .821 (.036) \\
		\texttt{GPT-4o-mini (temp0)} & .884 (.030) & .009 (.009) & .241 (.041) & .107 (.029) & .607 (.046) \\
		\texttt{GPT-4o-mini (multiple extraction)} & .634 (.046) & .009 (.009) & .232 (.040) & .000 (.000) & .170 (.036) \\
		\texttt{GPT-4o-mini (in-context)} & .902 (.028) & .000 (.000) & .446 (.047) & .009 (.009) & .741 (.042) \\
		\texttt{GPT-4o-mini (assert)} & .830 (.036) & .027 (.015) & .500 (.047) & .027 (.015) & .357 (.045) \\
		\hline
\end{tabular}


==> results/tables/latex_tables_subset_ci_inclusion.tex <==
% CI Inclusion Rate
\begin{tabular}{lccccc}
		\\
		\hline
		Model & Agree strongly & Agree & Neutral & Disagree & Disagree strongly \\
		\hline
		\texttt{GPT-4o-mini} & .107 (.029) & .000 (.000) & .250 (.041) & .071 (.024) & .375 (.046) \\
		\texttt{GPT-4.1} & .893 (.029) & .179 (.036) & .491 (.047) & .027 (.015) & .670 (.045) \\
		\texttt{GPT-5.4} & .973 (.015) & .009 (.009) & .402 (.047) & .000 (.000) & .955 (.020) \\
		\texttt{GPT-3.5-turbo} & .000 (.000) & .018 (.013) & .000 (.000) & .000 (.000) & .018 (.013) \\
		\texttt{gemma-3n-E4B} & .259 (.042) & .062 (.023) & .339 (.045) & .009 (.009) & .312 (.044) \\
		\texttt{Llama-3.3-70B} & .902 (.028) & .223 (.040) & .562 (.047) & .036 (.018) & .848 (.034) \\
		\texttt{Llama-3.1-8B} & .000 (.000) & .027 (.015) & .000 (.000) & .000 (.000) & .393 (.046) \\
		\texttt{Llama-4-Maverick} & .438 (.047) & .259 (.042) & .357 (.045) & .393 (.046) & .321 (.044) \\
		\texttt{Qwen3-A3B} & .366 (.046) & .018 (.013) & .045 (.020) & .232 (.040) & .241 (.041) \\
		\hline
\end{tabular}


==> results/tables/latex_tables_subset_success_rate.tex <==
% Pass rate at threshold 0.95 (proportion of propositions whose success rate exceeds it)
\begin{tabular}{lccccc}
		\\
		\hline
		Model & Agree strongly & Agree & Neutral & Disagree & Disagree strongly \\
		\hline
		\texttt{GPT-4o-mini} & .884 (.030) & .000 (.000) & .277 (.042) & .098 (.028) & .598 (.047) \\
		\texttt{GPT-4.1} & .902 (.028) & .188 (.037) & .491 (.047) & .036 (.018) & .661 (.045) \\
		\texttt{GPT-5.4} & .973 (.015) & .009 (.009) & .375 (.046) & .000 (.000) & .955 (.020) \\
		\texttt{GPT-3.5-turbo} & .241 (.041) & .071 (.024) & .009 (.009) & .009 (.009) & .250 (.041) \\
		\texttt{gemma-3n-E4B} & .429 (.047) & .071 (.024) & .804 (.038) & .009 (.009) & .464 (.047) \\
		\texttt{Llama-3.3-70B} & .893 (.029) & .223 (.040) & .536 (.047) & .036 (.018) & .848 (.034) \\
		\texttt{Llama-3.1-8B} & .000 (.000) & .027 (.015) & .000 (.000) & .000 (.000) & .357 (.045) \\
		\texttt{Llama-4-Maverick} & .571 (.047) & .286 (.043) & .339 (.045) & .411 (.047) & .339 (.045) \\
		\texttt{Qwen3-A3B} & .902 (.028) & .045 (.020) & .071 (.024) & .259 (.042) & .536 (.047) \\
		\hline
\end{tabular}

